Brownian motion on stationary random manifolds

We introduce the notion of a stationary random manifold and develop the basic entropy theory for it. Examples include manifolds admitting a compact quotient under isometries and generic leaves of a compact foliation. We prove that the entropy of an ergodic stationary random manifold is zero if and only if the manifold satisfies the Liouville property almost surely, and is positive if and only if it admits an infinite dimensional space of bounded harmonic functions almost surely. Upper and lower bounds for the entropy are provided in terms of the linear drift of Brownian motion and average volume growth of the manifold. Other almost sure properties of these random manifolds are also studied.

==> leaffunction.tex <==
\chapter{The leaf function of compact foliations}

\section{Introduction}\label{introduction}

\input{leaffunction/introduction.tex}

\section{Examples of leaf functions}\label{definitionsandexamplessection}

\input{leaffunction/definitionsandexamples.tex}

\section{Regularity of leaf functions}\label{maintheorems}

\input{leaffunction/compactnessandsemicontinuity.tex}

\section{Uniformly bounded geometry}\label{uniformlyboundedgeometrysection}

\input{leaffunction/spaces.tex}

\section{Smooth precompactness}\label{precompactness}

\input{leaffunction/precompactness.tex}

\section{Curvature and injectivity radius}\label{closedness}

\input{leaffunction/closedness.tex}

\section{Smooth convergence and tensor norms}\label{topology}

\input{leaffunction/topology.tex}

\section{Bounded geometry of leaves}\label{leafgeometrysection}

\input{leaffunction/leafgeometry.tex}

\section{Covering spaces and holonomy}\label{holonomysection}

\input{leaffunction/holonomy.tex}

\section{Convergence of leafwise functions}\label{leafwiseconvergencesection}

\input{leaffunction/leafwiseconvergence.tex}

==> section1/chapter1.tex <==

\chapter{Liouville properties and Zero-one laws on Riemannian manifolds}

\section*{Introduction}

\input{chapter1/introduction.tex}

\section{Brownian motion and the backward heat equation}

\input{chapter1/tail.tex}

\section{A bounded backward heat solution}

\input{chapter1/backward.tex}

\section{Steadyness of Brownian motion}

\input{chapter1/zerotwo.tex}

\section{Mutual information}

\input{chapter1/information.tex}


